Color: A Framework for Applying Graph Coloring to Subgraph Cardinality Estimation

Graph workloads pose a particularly challenging problem for query optimizers. They typically feature large queries made up of entirely many-to-many joins with complex correlations. This puts significant stress on traditional cardinality estimation methods which generally see catastrophic errors when estimating the size of queries with only a handful of joins. To overcome this, we propose COLOR, a framework for subgraph cardinality estimation which applies insights from graph compression theory to produce a compact summary that captures the global topology of the data graph. Further, we identify several key optimizations that enable tractable estimation over this summary even for large query graphs. We then evaluate several designs within this framework and find that they improve accuracy by up to 10$^3$x over all competing methods while maintaining fast inference, a small memory footprint, efficient construction, and graceful degradation under updates.

==> 5-updates.tex <==
\section{Handling Updates}
\label{sec:updates}

\textcolor{red}{Kyle: At a high level, this section breaks with the previous sections because it specifically handles the average degree statistic. We need to call this out explicitly somewhere early or the reader will be confused. Every estimator will inherently require its own update algorithms, so I think this focus is okay. It just requires the framing to be a bit more like "this is an example of how an estimator can handle updates" and less "this is how updates are handled under our framework". Additionally, this section is lightly hampered by a poor discussion of labels in earlier sections, so there's not a lot of good notation around that. I think the fix might be to add a label argument to $\psi$ and $\tau$ when talking about labeled graphs, but that will need to be propagated to the above sections. Let me know if you want to meet about this part.}


\emph{Motivation}. Practically, databases generally receive many updates over the course of their lifetimes. Thus, we need a way to efficiently and accurately update our lifted graph with incoming data to maximize the time before it becomes outdated and a new set of statistics must be built. We define a summary update function to accommodate these changes without touching $G$. \textcolor{red}{Kyle: I like this paragraph. Maybe drop the first sentence (it's a given that updates are important) and expand the second one into two sentences because I think it captures the core of our approach to updates (gracefully degrade between very intermittent rebuilds). Nit: "Thus" is basically never necessary. I have a habit of adding too many "[therefore/further/so/etc],"'s at the beginning of sentences, but they're often not really necessary.}


\begin{definition}
    \label{def:summary-update}
    Given a data graph $G$, a lifted graph $F = (G_F, \psi, \tau)$, and update $\theta$, we define the summary update function as follows where $F'$ is the updated lifted graph,
    \begin{align*}
         F' = \delta (F, \theta)
    \end{align*}
    $\theta$ can either describe an edge to create between existing vertices or a new vertex to add with a corresponding label set $L$:
    \begin{itemize}
        \item $\theta_E = (v_1, v_2, L)$ where $v_1 \in G_V, v_2 \in G_V, $
        \item $\theta_V = (v, L)$
    \end{itemize}
\end{definition}
\textcolor{red}{Kyle: I like the update function notation a lot, but I would move the definition of an update above into its own definition. This will give you a sentence or two to describe the kind of updates that we allow. Then, once the problem setting is clear, go ahead and define the update function as you did $\delta(F, \theta) = F'$ where it takes in a lifted graph \& update and outputs an updated lifted graph. Plus, with the updates already defined, you can move the below discussion into that definition potentially.}


Depending on the type of $\theta$, the definition of $\delta$ can change, affecting different parts of the lifted graph for edge updates $\delta_E$ or vertex updates $\delta_V$:
\begin{align*}
    \delta &= \begin{cases}
    \delta_E, & \text{$\theta \in \theta_E$} \\
    \delta_V, & \text{$\theta \in \theta_V$}
    \end{cases}
\end{align*}

\subsection{Edge Updates}
The edge update function $\delta_E$ only affects edge statistics in a lifted graph:
\begin{align*}
    \delta_E(\theta_E, (G_F, \psi, \tau)) = F' = (G_F, \psi, \tau')
\end{align*} 
\textcolor{red}{Kyle: I think you can drop this equation and just say in the text that this kind of update only affects $\tau$.}
We need to adjust the edge degree statistics to account for the addition of a new edge. For example, if $\theta_E = (v_1, v_2, L)$ and $\sigma (v_1) = C_1, \sigma(v_2) = C_2$, for the average degree $\tau(C_1, C_2) = S_{l_{AvgDeg}}$, the result of the update, $\tau'(C_1, C_2)=S_{l_{AvgDeg}}'$, is represented by:\\
\begin{align*}
    S_{l_{AvgDeg}}' = \frac{(S_{l_{AvgDeg}} * \psi (C_1) + \frac{|(e|\lambda (e_1) = L, e \in E_F, e=(e_1, e_2)|}{|E_F|})}{\psi(C_1)} \forall L \in \mathbb{L}_{v_2} \\
\end{align*}
\textcolor{red}{Kyle: I think this is a good start but needs some cleaning up. I would drop $S_{l_{AvgDeg}}$ and instead always refer to $\tau(C_1,C_2)$ and $\tau'(C_1,C_2)$, or potentially $\tau_{AvgDeg}(C_1,C_2)$ if that feels clearer. Also, drop the "for example" above, if we've already explained that we're talking about $\ell_{AvgDeg}$ at the start of the section, then this can just be framed as providing a formal definition for $\delta_E$. Nit: Sets are denoted using $\{\}$ not $()$.}

Since the IDs of the vertices are given by $\theta_E$, we can use $\sigma$ to find their colors \textcolor{red}{Kyle: This is another bit that's not discussed in the prior notation really, and maybe it should be. We need to talk about the use of cuckoo filters somewhere because this is how we keep $\sigma$ around.}, but we the labels of those vertices' are unknown. So, when an edge is added to the graph, we update the degree statistics corresponding to the colors that its vertices belong to. However, instead of just updating the degree statistics for an arbitrary vertex label, we distribute the value of the edge across all degree statistics for each possible landing vertex label, scaling accordingly to the number of existing edges with the label. Overall, the average degree increases with the addition of an edge to the lifted graph.
\textcolor{red}{Kyle: I like this discussion a lot, and it'll be super clear to the reader once we have a better description of how labels are handled earlier in the paper.}

\subsection{Vertex Updates}
The vertex update function $\delta_V$ affects the stored edge statistics and the color sizes in a lifted graph:
\begin{align*}
    \delta_V(\theta_V, (G_F, \psi, \tau)) = F' = (G_F, \psi', \tau')
\end{align*}
During a vertex update, we cannot guarantee what its degrees will be like after subsequent edge updates, so it is difficult to choose a color with edge statistics that resemble the new vertex. Instead, for $\theta_V = (v, L)$, we can choose to add the vertex $v$ to the largest existing color:
\begin{align*}
    \sigma (v) = C_{largest} \; | \; \psi (C_{largest}) = max(\psi(c) \forall c \in C)
\end{align*}
The largest color will have the highest variance in its statistics \textcolor{red}{Kyle: This isn't necessarily true because the largest color could have all identical nodes. But, adding to the largest color does have the smallest impact on the average degree statistics.}, so we can preserve the higher quality information in other colors while gradually updating the statistics that belong to the largest color. (Right now doing tests to see what performance is like if we add it to its own color instead because that seems more intuitive...) \textcolor{red}{<--- Kyle: Always add these comments in the "textcolor" environment. We really don't want to miss one and leave it in when we submit.}
After choosing $\sigma(v) = c$, we can adjust $\psi$ by:
\begin{align*}
    \psi'(c) = \psi(c) + 1
\end{align*}
A vertex update will also affect the edge degree statistics. For example, for the average degree statistic $S_{l_{AvgDeg}}$, if $\theta_V = (v, L)$ and $\sigma(v) = c$, then: 
\begin{align*}
    \tau'(c, c_i) = S_{l_{AvgDeg}}' = \frac{S_{l_{AvgDeg}} * \psi (c)}{\psi'} \; \forall \; c_i \in C\\
\end{align*}
\textcolor{red}{Kyle: Nit: remove $S_{l_{AvgDeg}}$ as above.}
A new vertex has no edges, so it will decrease the average degree for the color it belongs to (essentially adding a 0 to the set that is being averaged). 
\subsection{Cycle Closing Probability}
The lifted graph contains statistics about the cycle-closing probability for existing nodes and edges, but additions to the graph change this probability. To account for this, we make an adjustment to the $\omega^\circ_{CCP}$ function. We treat the closure of the paths with an update edge as its own independent event, then continue to calculate the probability of at least one cycle-closing event occurring. For a set of edge updates, $\mathbb{S}_{\theta E}$:
\begin{align*}
    \omega^\circ_{CCP}(\pi, e_i|e_1,\ldots,e_{i-1}) &= 1 - \prod_{P\in\bf{P}}(1- \tau_{\mathcal{P}}(\pi(e_i))(1-\frac{|\mathbb{S}_{\theta E}|}{|V_F|^2})(P)
\end{align*}
Note also that since $\delta_E$ and $\delta_V$ adjust $\tau$ and $\psi$ in a lifted graph $F$, the independent cycle likelihoods are adjusted as well. \textcolor{red}{Kyle: I'm not sure if the reader will know what "independent cycle likelihoods" means...}


% \subsection{Experiments}
% \textcolor{red}{Kyle: This discussion will go in the "Evaluation" section.}

% Protocol: Choose a number of edges to initialize a graph with and build a summary based on those starting edges. Then, update the graph with the leftover nodes, then edges from the original data graph and run the queries on the resulting summary.


% With increasing updates, the performance of the lifted graph summary is expected to degrade towards that of the hash coloring, with the colors gradually losing meaning in their stored statistics. With our method we do not need to create a new summary every time the database is updated and instead wait until the number of updates is expected to begin impacting the quality of estimates.


==> 7-related_works.tex <==


\section{Related Work}
Cardinality estimation in graph databases is a growing source of attention. There are many competing methods that should be discussed. 

An important class of cardinality estimation methods are those which utilize machine learning. Learned query-driven methods like \cite{DBLP:journals/dase/ZhaoHYR23} use a subset of query graphs to train a model while learned data-driven methods like \cite{DBLP:journals/pacmmod/WuNAKM23, DBLP:journals/vldb/ZhaoYLZR23} aim to identify patterns in the data. While machine learning methods boast relatively high accuracies, they can have slower training times and are dependent on the quality of their training sets \cite{DBLP:journals/pacmmod/WuNAKM23, DBLP:journals/dase/ZhaoHYR23, DBLP:journals/vldb/ZhaoYLZR23}.

Some non-learning methods like \cite{DBLP:journals/tkdd/ChenL18, DBLP:conf/sigmod/KimKFH21} have adopted online sampling, using various techniques to sample from the database during processing like random walks in \cite{DBLP:journals/tkdd/ChenL18}. While these methods achieve high efficiency and accuracy after using their generated samples, directly obtaining samples from the database can be an expensive operation that faces issues in distributed or disk-based settings. 

Many summary-based methods utilize offline preparation, generating summary to avoid expensive database accesses when processing queries. Like \cite{DBLP:conf/icde/NeumannM11, DBLP:conf/www/StefanoniMK18, DBLP:journals/complexity/ShanLJLS21, DBLP:conf/edbt/WortelerRCG22, DBLP:journals/pvldb/SunSC0H20, DBLP:conf/sigmod/WangH000022}, our method preprocesses data offline before handling queries. These methods differ by the way they form their lifted statistics. For example, \cite{DBLP:conf/www/StefanoniMK18} groups nodes with similar node labels and edge connections while \cite{DBLP:journals/complexity/ShanLJLS21} groups connected nodes with the same labels. Compared to these methods, we offer faster runtimes and higher accuracies, as demonstrated by our experiments. 
% \textcolor{red}{We will hopefully be much faster than many of these.}. The main drawback, however, is the inability to efficiently add new data to the database. \textcolor{red}{We'll need to have a good response to this before bringing it up as a drawback. So, maybe drop unless we have a method for handling updates.}


% \textcolor{red}{Tighten here.} . These methods can demonstrate great efficiency and accuracy as well. However, directly sampling from the data graph usually is not preferred since it can be an expensive operation. \textcolor{red}{Here, we should definitely mention that these methods face major issues when in distributed or disk-based settings. In these settings, the random accesses from walk-based sampling methods can cause bigger issues. Also, calling it efficient and expensive is a bit counterintuitive, so it would require further explanation.}

Cardinality estimation is not exclusive to graph databases. In the relational setting other popular methods include \cite{DBLP:conf/sigmod/CaiBS19, DBLP:journals/tods/LiWYZ19, DBLP:journals/pvldb/VengerovMZC15, DBLP:conf/sigmod/ZhaoC0HY18}. These methods are applicable to graph databases but may struggle with the higher frequency of joins in graph queries. If possible, some of these methods have been adapted to graph settings. For example, \cite{DBLP:conf/sigmod/KimKFH21} utilizes the random walk method described in \cite{DBLP:journals/tods/LiWYZ19}.
% \textcolor{red}{Because graph queries are a subset of relational queries, these methods will always be applicable. Instead, I think the key is that graph queries involve many more joins and these methods often have trouble as the number of joins increases.}.

Finally, there are also methods that combine existing approaches to cardinality estimation, such as \cite{DBLP:journals/sigmod/ChenHWSS23, DBLP:journals/tkde/LeeuwenFY23}. Our approach could be seen as a promising candidate to further improve the accuracy of these methods.


% \textcolor{red}{Summary: I think this was a great first draft. The broad breakdown of methods makes sense, and the literature review seems pretty detailed. At a high level, I would keep an eye on writing concisely, although this often does just come from rounds of edits. Also, keep an eye on combinations of statements that seem counter intuitive to a reader at a first glance, these will always require justification, citation, or explanation. Lastly, we'll have to do more edits on this after the experiments to alter the framing of it a bit towards our strengths.}

% \begin{itemize}
%     \item FactorJoin: A New Cardinality Estimation Framework for Join Queries [6]
%     \begin {itemize}
%         \item Combines join-histogram method (for joins) with learning-based methods to capture attribute correlation
%         \item scans table in a db and builds conditional distributions offline
%         \item when join query comes, translated into factor graph model using distributions
%     \end {itemize}
%     \item CharacteristicSets [G-Care 30] [7]
%     \item SumRDF (Estimating the Cardinality of Conjunctive Queries over {RDF} Data Using Graph Summarisation)[G-Care 38] [8]
%     \item Supergraph Topology Feature Index for Personalized Interesting Subgraph Query in Large Labeled Graphs [9]
%     \begin {itemize}
%         \item Uses isotype structure graph compression
%         \item replace data graph with supergraph topology feature index, then partition index logically
%         \item new subgraph query approach proposed (multidimensional filtering, upper bound value matching, optimizational join method to filter false subgraph candidates)
%     \end {itemize}
%     \item Cardinality Estimation using Label Probability Propagation for Subgraph Matching in Property Graph Databases [10]
%     \begin {itemize}
%         \item Uses information about node labels and relationship types to generate label probability
%     \end {itemize}
%     \item IMPR (Mining Graphlet Counts in Online Social Network) [11]
%     \item Combining Sampling and Synopses with Worst-Case Optimal Runtime and Quality Guarantees for Graph Pattern Cardinality Estimation [12]
%     \begin {itemize}
%         \item Hybrid cardinality estimation using both sampling and synopses
%         \item random walk with intersection for sampling, branching to reduce variance, extraction and indexing of tangled patterns as synopses
%         \item used during online estimation
%     \end {itemize}
%     \item RapidMatch [13]
%     \begin {itemize}
%         \item shows that complexity in exploration-based query searches match worst-case optimal join
%         \item Subgraph query processing framework that combines exploration and joins
%     \end {itemize}
%     \item Learning with Small Data: Subgraph Counting Queries [14]
%     \begin {itemize}
%         \item Gaussian Process trained by meta learning algorithm on small training data
%         \item Obtain model to encode data and pattern graphs and capture prior
%         \item Handle pairs (g,p), the data-pattern pair
%     \end {itemize}
%     \item A Learned Sketch for Subgraph Counting. [15]
%     \begin {itemize}
%         \item Propose active learned sketch for subgraph counting
%         \item Sketch is learned by neural network regression model
%         \item Active learner performs model updates based on new queries
%     \end {itemize}
%     \item Bound Sketch (Pessimistic cardinality estimation: Tighter upper bounds for intermediate join cardinalities)  [G-Care 8] [16]
%     \item WanderJoin [G-Care 23] [17]
%     \item CorrelatedSampling (Join size estimation subject to filter conditions) [G-Care 41] [18]
%     \item Join Sampling with Upper Bounds (Random sampling over joins revisited) [G-Care 44] [19]
%     \item Accurate summary-based cardinality estimation through the lens of cardinality estimation graphs. [20]
%     \begin {itemize}
%         \item Looks at optimistic vs pessimistic estimators
%         \item Models estimators as picking bottom-to-top paths in cardinality estimation graphs
%         \item different paths for different query structures
%     \end {itemize}
%     \item A General Cardinality Estimation Framework for Subgraph Matching in Property Graphs [21]
%     \begin {itemize}
%         \item obtain estimates for subqueries, extend set, combine into single estimate
%         \item different existing approaches can be used in one of the phases
%         \item can estimate query patterns without property constraints with small pattern synopses
%         \item property constraints require new techniques that capture correlation between property constraints and topology
%     \end {itemize}
%     \item Neural Subgraph Counting with Wasserstein Estimator [22]
%     \begin {itemize}
%         \item  Generates substructures from data graph for queries, then uses estimator that computes representations and estimates subgraph counts
%         \item Design Wasserstein discriminator to minimize Wasserstein distance between query and data graphs
%     \end {itemize}
% \end{itemize}

==> response.tex <==
{\large
We thank the reviewers for their insightful comments and their recommendation to \textit{accept with shepherding}. We were able to incorporate all the changes corresponding to your comments, which significantly improved our paper. This involved adding new theory results, extending the empirical study in the experiments section and improving the clarity of the writing. For ease of comprehension, we color-coded our changes by reviewer, both here and in the manuscript text.

\hspace*{\fill}---The Authors

\rone{
\textbf{Reviewer One}
\begin{itemize}
    \item W1 (\textit{Extending theoretical bounds on stable coloring to quasi-stable coloring}): We have added a theoretical analysis of the error bound due to quasi-stable coloring in Section~\ref{subsec:stable-colorings}.
\end{itemize}
}

\rtwo{\textbf{Reviewer Two}
\begin{itemize}
    \item W1 (\textit{Error metric definition}): We have clarified the definition of the error metric we use in the experiments and the motivation behind it, in Section \ref{subsec:accuracy}.
    \item W2 (\textit{Timeout choice}): We now discuss the choice of one minute timeout, with reference to matching timeouts in the literature, in Section \ref{subsec:inference-latency}. We note that our method runs well below the timeout---we set it to one minute to accommodate the slower baseline methods.
    \item W3 (\textit{Intuition for resiliency to undersampling}): We add the intuition behind why our method is resilient to sampling failure, unlike baseline methods, in Section~\ref{subsec:estimator-failure}.
\end{itemize}
}

\rthree{\textbf{Reviewer Three}
\begin{itemize}
    \item W1 (\textit{Comparasion  with additional baseline methods}~\cite{DBLP:journals/vldb/ZhaoYLZR23, DBLP:conf/sigmod/WangH000022, DBLP:journals/pvldb/ShinSPH24}): We have updated the paper to take into account the three related baseline methods the reviewer brought to our attention. The system \textsc{lss}, introduced in the paper ``A Learned Sketch for Subgraph Counting''~\cite{DBLP:journals/vldb/ZhaoYLZR23} is the most comparable. We believe \textsc{lss} is a good representative for the machine learning-based approaches. We benchmark it and add it to all relevant experiments figures throughout Section \ref{sec:evaluation}. See the updated Figures~\ref{fig:relative-error}, \ref{fig:inference-time}, \ref{fig:build-time}, \ref{fig:statistics-size} and their accompanying discussion.\\ Meanwhile, the approaches in ``Neural Subgraph Counting with Wasserstein Estimator''~\cite{DBLP:conf/sigmod/WangH000022} and "Cardinality Estimation of Subgraph Matching: A Filtering-Sampling Approach"~\cite{DBLP:journals/pvldb/ShinSPH24} address subgraph isomorphism (rather than homomorphism). As such, they cannot be directly evaluated with the subgraph homomorphism benchmarks we use. Consequently, we include a discussion of these two approaches in introduction to Section \ref{sec:evaluation}.
\end{itemize}
}
}
